Where to Drop Sensors from Aerial Robots to Monitor a Surface-Level Phenomenon?

We consider the problem of routing a team of energy-constrained Unmanned Aerial Vehicles (UAVs) to drop unmovable sensors for monitoring a task area in the presence of stochastic wind disturbances. In prior work on mobile sensor routing problems, sensors and their carrier are one integrated platform, and sensors are assumed to be able to take measurements at exactly desired locations. By contrast, airdropping the sensors onto the ground can introduce stochasticity in the landing locations of the sensors. We focus on addressing this stochasticity in sensor locations from the path-planning perspective. Specifically, we formulate the problem (Multi-UAV Sensor Drop) as a variant of the Submodular Team Orienteering Problem with one additional constraint on the number of sensors on each UAV. The objective is to maximize the Mutual Information between the phenomenon at Points of Interest (PoIs) and the measurements that sensors will take at stochastic locations. We show that such an objective is computationally expensive to evaluate. To tackle this challenge, we propose a surrogate objective with a closed-form expression based on the expected mean and expected covariance of the Gaussian Process. We propose a heuristic algorithm to solve the optimization problem with the surrogate objective. The formulation and the algorithms are validated through extensive simulations.

==> OLD/old.tex <==
\section{PROBLEM FORMATION: Stochastic Case}


A UAV is equipped with a size $B$ battery and $n$ sensors, denoted by the set $\bm{N}=\{1,2,\ldots, N\}$. The mission of UAV is to plan an optimal route $\tau^*$ and airdrop the sensors to an area on the ground to measure $m$ distinct Points of  Interest (PoIs) at a designated end time $t_{end}$. We assume that UAV can drop the sensors at some discretized locations in the air and all the possible airdrop locations form a connected graph $G=(V_{\text{airdrop}}, E)$, where $V_{\text{airdrop}}$ denotes the collection of all possible airdrop locations and $E$ denotes the set of possible transitions between airdrop locations. Each edge $e_{ij}$ has a corresponding cost $c_{ij} \in C \subset \mathbb{N}$. The cost function is given by 

 \begin{equation} c_{ij} = 
     \begin{cases}
     d_{ij}/s & \text{ if node $i$ and node $j$ are connected} \\ 
     \infty& \text{ else} 
    \end{cases}
\end{equation}
where $d_{ij}$ is the flight distance between node $i$ and node $j$ and $s$ is the constant spend of the UAV. The UAV can travel between the nodes on the graph $G$ and the distance must not exceed the UAV’s battery capacity $B$.

Let us first consider \todo{the deterministic case}, that is, we can predict the exactly sensor locations at some vertices in $V_{\text{sensor}}$. In this case, each location is only allowed to drop one sensor.

A good placement would maximize the different between $H(\bm{Y}_{\scaleto{\text{PoIs}}{4pt}})$ and $H(\bm{Y}_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{Y}_{A})$, i.e., reduce the uncertainty at $V_{\text{PoIs}}$. Mathematically, we want to find
\begin{equation}
    A^* = \argmax_{A \subseteq V_{\text{sensor}}}  H(\bm{Y}_{\scaleto{\bm{V}_{\text{PoIs}}}{4pt}}) - H(\bm{Y}_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{Y}_{A}).
\end{equation}
\todo{need to check submodularity}
%Submodularity issues in value-of-information-based sensor placement

\begin{itemize}
    \item \todo{show the objective is approximately submodular using approximate submodular ratio}
    \item \todo{enlarge the PoIs to include all possible sensor landing locations}
\end{itemize}


Now, we consider the stochastic case. Due to the disturbances of the wind, the landing position $\bm{x}_v$ when a sensor is dropped at the node $v$ is stochastic. We assume that $\bm{x}_v$ has a Gaussian distribution with a known mean $\mu_v$ and variance $\sigma_v^2$. 

The expected conditional entropy $\mathbb{E} \left [ H(\bm{Y}_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{Y}_{A})  \right ]$ can be computed as 
\begin{align}\label{eq:expected_conditional_entropy}
    &\int \int H(y_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{y}_{A}) p(\bm{y}_A \mid \bm{x}_{A})p(\bm{x}_{A}) ~\text{d} \bm{y}_{A} ~\text{d} \bm{x}_{A} \\
    =& \int H(y_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{y}_{A}) p(\bm{x}_{A}) ~\text{d} \bm{x}_{A}
\end{align}

The goal is to select $N$ vertices in graph $G$ to drop sensors to reduce the uncertainty of PoIs. We denote the set of PoIs as \st{${\mathcal{P}}$} $ V_{\text{POIs}}$. Mathematically, 
\begin{align}
    \max_{A \subseteq V} H(\bm{Y}_{\scaleto{\text{PoIs}}{4pt}}) - \mathbb{E} \left [ H(\bm{Y}_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{Y}_{A})  \right ] ,
\end{align}
\iffalse
where $H(f(\mathcal{P}))$ is the entropy of the prior distribution (Gaussian) of values of PoIs and can be computed analytically; $\mathbb{E} \left [ H(f_{\mathcal{P}} \mid \mathcal{L}(A)) \right ]$ denotes the expected entropy of the posterior distribution of values of PoIs when a set of sensors $A$ is dropped. 

The challenge is to compute $\mathbb{E} \left [ H(f_{\mathcal{P}} \mid \mathcal{L}(A)) \right ]$.
we need to solve the following integral:
\begin{equation}\label{problem:main_original}
    \int \int H(f_\mathcal{P} \mid \mathcal{L}(A), y)p(y \mid \mathcal{L}(A))p(\mathcal{L}(A)) ~\text{d} y ~\text{d} \mathcal{L}(A).
\end{equation}
\fi

\todo{Eq. \eqref{eq:expected_conditional_entropy}  is in general intractable since the locations $\bm{x}$ will show in the kernel.} We have to resort to approximation. The challenge here originates from the stochasticity of the landing positions of the sensors. If the landing position is deterministic, the posterior distribution is still Gaussian as shown in \todo{XX}, and the second term in Eq. \eqref{problem:main_original} can be computed easily. Therefore, the key to approximating the stochastic version of the problem is how to deal with the input uncertainty. One observation is that the uncertainty on the output side can be easily dealt with as shown in XX. The idea of approximating the problem \todo{XX} is to `propagate' the uncertainty of the input to the output such that the resulting problem is similar to problem \todo{XX} but with a different output uncertainty. 


\section{PROBLEM FORMATION: Deterministic Case}
In this section, we address the offline path planning and airdrop scheduling problem for UAV sensors airdrop missions. Our objective is to determine the optimal path, drop points, and drop angles considering constraints of airdrop dynamics, underwater conditions, and battery size. By formulating the mission as an offline optimization problem, we aim to maximize mission efficiency and sensor coverage.

\subsection{Path Planning for UAV}

% 1. N < M; more POIs than sensors
%   Extra lemma that says ``there exists an optimal solution with exactly N (or N+1) vertices that are all sensor nodes.'' Submod Orienteering.
% 2. N >= M; more sensors than POIs
%   2A. B is enough to visit all POIs: TSP
%   2B. B is not enough to visit all POIs: Submod Orienteering
%
% We can handle 1 and 2B with the same algorithm
%
% O1: minimize the sum of distance between POI and nearest sensor
% O2: maximize the sum of the reciprocal of the distance between POI and nearest sensor: submodular
% O3: maximize the mutual information

% I still dont understand why do we need more sensors in the deterministic case. 
% Example: 2 POIs and 3 sensors
% 2A. If B is enough, we can find 2 optimal locations to drop the sensors, namely node A and B
% 2B. If B is not enough and we find 3 locations to drop the sensors, namely A', B', and C', such that total traveling cosst < B
%     From the cost function J, we know that, for each POI, the cost depends only on the closest dropped sensors.
%     Ie, POI 1 depends on A' and POI 2 depends on B'. There is a  redundant sensor C'. 
%     We always can remove the sensor C' without changing the total traveling cost B.
%     Therefore, we need at most M sensors.



 
 Given an environment $\varepsilon \in  \mathbb{R}^3$, an UAV has $n$ sensors, denoted by the set $\mathbf{N} = (1,2,...,N)$.  The UAV's mission is to deploy these sensors to $m$ distinct Points of Interest (POIs) at a designated end time $t_{end}$, denoted by the set $\mathbf{M} = \{1,2,...,M\}, n \leq m$. The coordinates of targets are represented as $(x_i, y_i,z_i)$. The environment is represented by a discrete undirected graph $\mathbf{G} = (V,E,C)$, where $V= (v_1,v_2,v_3, ... v_K)$ represents the nodes or potential travel points, and $E$ represents the edges connecting these nodes.  $v_i = (x,y) \in \mathbb{R}^2 \subset \varepsilon$ is a coordinate in the 2D map of the environment. The edge $e_{ij} \in E$ connects the node $i$ and the node $j$ with the cost $c_{ij} \in C \subset \mathbb{N}$. The cost $c_{ij}$ represents the needed time traveling from the node $i$ to node $j$. The cost function is given by 

 \begin{equation} c_{ij} = 
     \begin{cases}
     d_{ij}/s & \text{ if node $i$ and node $j$ are connected} \\ 
     \infty& \text{ else} 
    \end{cases}
\end{equation}
where $d_{ij}$ is the flight distance between node $i$ and node $j$ and $s$ is the constant spend of the UAV. The UAV can travel from node $i$ to $j$ along the edge $e_{ij}$ for any given t. For example, if the UAV leaves node $i$ at time $t$, it arrives the node $j$ at time $t+c_{ij}$. The time is discretized as $[t_0, t_0+1, t_0+2,..., t_{end}]$. 

At a high level, the problem studied in this paper is stated below.

\textbf{Problem}. Given an discrete undirected graph $\mathbf{G}=(V,E,C), n$ sensors, and $m$ target location, find the optimal route $\tau^* = (\tau_1, \tau_2, ..., \tau_w), \tau_i =(t,v_j) \in [t_0,t_{end}] \times V $, the optimal drop points $\delta^*=(\delta_1,\delta_2,...,\delta_j) and \delta_i=(t,v_j) \in [t_0,t_{end}] \times V$ to minimize the cost function, such that 

\begin{equation}
    \begin{aligned}
        \min_{\tau, \delta, \theta} J = \min_{\tau, \delta, \theta} \sum_{i=1}^M \min_{j \in [1,...,N]}  d(p_j(t_{end}),q_i)   \\
        \text{s.t.} \sum_{k = 1}^{w-1} c_{v(\tau_i), v(\tau_{i+1})} \leq B \\
        \delta_a \neq \delta_b, \forall a,b \in 1, ... ,M \\
        p_j(t) = f(g(\delta_j,\theta_j, z_{UVA})) \\
        \tau_1 = (t_0, v_1)  \text{and}  \tau_w = (t_{end}, v_1)
    \end{aligned}
\end{equation}

where the function $d(\cdot,\cdot)$ is the distance of two points, $p_j(t)$ is the position of the $j$ th sensor at time $t$, $q_i$ is the  position of target $i$, $B$ is the Battery capacity, the function $f$ models the dynamics of underwater object, the function $g$ models the dynamics of airdrop, and $z_{UVA}$ is the constant altitude parameter of the UAV. 

The cost function represents the sum of the minimum distances between each deployed sensor's position $p_j(t_{end})$ and its respective target location $q_i$. The optimization is subject to various constraints. The total distance traveled in the route must not exceed the UAV's battery capacity $B$. The drop points must be distinct to avoid overlap, and the dynamics of both the underwater objects and the airdrop process are considered through the functions $f$ and $g$, respectively. The constant altitude parameter of the UAV is denoted as $z_{UAV}$.

\textcolor{red}{New Model}
\textcolor{red}{
    \begin{equation}
        \begin{aligned}
            \max_{\tau, \delta, \theta} J = \max_{\tau, \delta, \theta} \sum_{i=1}^M \max_{j \in [1,...,N]} \frac{1}{d(p_j(t_{end}),q_i)} \\
            \text{s.t.} \sum_{k = 1}^{w-1} c_{v(\tau_i), v(\tau_{i+1})} \leq B \\
            \delta_a \neq \delta_b, \forall a,b \in 1, ... ,M \\
            p_j(t) = f(g(\delta_j,\theta_j, z_{UVA})) \\
            \tau_1 = (t_0, v_1)  \text{and}  \tau_w = (t_{end}, v_1)
        \end{aligned}
    \end{equation}
}

\begin{align} 
E[J] &= \sum_{i=1}^M E[\max_{j \in [1,...,N]} \frac{1}{d(p_j(t_{end}),q_i)}] \\
&\geq \max_{j \in [1,...,N]} E[\frac{1}{d(p_j(t_{end}),q_i)} ]\\
OPT &\geq LOPT\\
ALG &\geq \dfrac{1}{\alpha} LOPT\\
\end{align}


%\subsection{Deployment Angel}
%In this paper, the drop angle is discretized into $H$ directions. The set of possible drop angles, denoted as $A= \{0,\frac{2\pi}{H}, \frac{4\pi}{H}, ..., \frac{(H-1)\pi}{H}\}$. The UVA can decide to drop the sensor following the drop angel at any given node. By considering the dynamics of airdrop, the drop angle plays a crucial role in determining the terminal position when it entries into the water.
 
\subsection{Dynamics of Airdrop}
We still need a dynamics model for this part.
%\subsection{Dynamics of Underwater Object}
We still need a dynamics model for this part.

\subsection{NP Hard Problem}

\section{PRELIMINARIES}
\subsection{Notations}\label{sec:notation}
\begin{itemize}
    \item scalar: $x$ $X$ not bold and Roman
    \item vector: $\bm{x}$ $\bm{X}$ bold and Roman
    \item random variable: $\mathbf{x}$ $\mathbf{X}$ math bold  
\end{itemize}

\subsection{Gaussian Process}
The Gaussian Process (GP) generalizes multivariate Gaussian distribution to the case of multiple random variables. It can be used for either classification or regression (GPR) tasks in machine learning \todo{XX}. In the robotics community, GP representation is widely used in applications that involve uncertainty \todo{XXX}, since the GP can naturally provide a closed-form uncertainty quantification using proper kernel functions. 
In this paper,  we use GP to approximately represent a spatial function $f(\bm{x}): \mathbb{R}^{ 2} \to \mathbb{R}$ (e.g., temperature field) of a task area, i.e.,
\begin{equation}
    {f}(\bm{x}) \sim \mathcal{GP}(\mu(\bm{x}), k(\bm{x}, \bm{x}^{\prime})),
\end{equation}
where $\mu(\bm{x})$ is the prior mean function and we make the standard assumption that $\mu(\bm{x})=0$ as in \todo{XX}; and the $k(\bm{x}, \bm{x}^{\prime})$ is the positive-definite kernel function. 

When we deploy sensor at the locations $\bm{x}$, we do not have access to function value ${f}(\bm{x})$ directly, but only noisy observation 
\begin{equation}
    {y} = {f}(\bm{x}) + \epsilon,
\end{equation}
where $\epsilon \sim \mathcal{N}({0}, \sigma^2_{\epsilon})$ is the Gaussian Noise.  

Given a query point $\bm{x}_*$ and a data set $\mathcal{D}=\{\bm{x}_i, y_i\}_{i=1}^{\abs{\mathcal{D}}}$, the posterior distribution of $\bm{f}(\bm{x}_*)$ is : 
\begin{equation}
    p({f} \mid {\bm{x}_*, {X}, \bm{y}})=\mathcal{N}(\bar{{f}}, ~\text{Cov}({f})),
\end{equation}
where we denote the stacked $\bm{x}_i$  and ${y}_i$ as ${X} \in \mathbb{R}^{\abs{\mathcal{D}} \times 2}$ and $\bm{y} \in \mathbb{R}^{\abs{\mathcal{D}}}$, respectively;
\begin{equation}
    \bar{{f}} \coloneqq k(\bm{x}_*, {X})\left [ k({X}, {X}) + \sigma_{\epsilon}^2I \right]^{-1}\bm{y}
\end{equation}
is the mean at the point $\bm{x}_*$ and the covariance is 
\begin{equation}\label{eq:posterior_covariance_deterministic}
    \begin{aligned}
        \text{Cov}({f}) \coloneqq & k(\bm{x}_*, \bm{x}_*) \\
        -k(\bm{x}_*, X)^T & \left [ k(X, X) + \sigma_{\epsilon}^2I \right ]^{-1}k( \bm{x}_*, X).
    \end{aligned}
\end{equation}
It should be noted that the covariance function is independent of the measurement $\bm{y}$.


\subsection{Entropy and Mutual Information}
Consider the scenario shown in Fig. \textcolor{red}{XX}. There are two types of vertices: $V_{\text{PoIs}}$ denotes the set of points of interest in which we want to reduce the uncertainty; $V_{\text{sensor}}$ denotes the set of potential sensor dropping locations. The function value (a random vector) at the points of interest is denoted as  $\bm{f}_{\text{PoIs}}$. We want to reduce the uncertainty at $V_{\text{PoIs}}$
by dropping sensors to some vertices in $V_{\text{sensor}}$. 

Before dropping any sensor to $V_{\text{sensor}}$, the uncertainty at $V_{\text{PoIs}}$ can be quantified based on entropy using GP prior,
\begin{equation}
    H(\bm{f}_{\text{PoIs}}) = - \int p({f}_{\text{PoIs}}) \log p({f}_{\text{PoIs}}) d {f}_{\text{PoIs}}. 
\end{equation}

%We can get one analytical solution for this entropy.

After dropping sensors to a subset of vertices  $A \subseteq V_{\text{sensor}}$, one natural notion of uncertainty is the conditional entropy of $V_{\text{PoIs}}$, 

\begin{align}
    &H(\bm{f}_{\text{PoIs}} \mid X_A, \bm{y}_{A}) \\
    &= - \int p({f}_{\text{PoIs}}, y_{A}) \log p({f}_{\text{PoIs}} \mid \bm{x}_A, {y}_{A}) 
    d {f}_{\text{PoIs}} d {y}_{A} \\
    %\\&= - \int p(f_{\scaleto{V_{\text{PoIs}}}{4pt}}) \log p(f_{\scaleto{V_{\text{PoIs}}}{4pt}} \mid X_A, \bm{y}_{A}) 
    %d f_{\scaleto{V_{\text{PoIs}}}{4pt}} 
    &= - \int p({f}_{\text{PoIs}} \mid {y}_{A})  \log p({f}_{\text{PoIs}} \mid \bm{x}_A, {y}_{A}) p({y}_{A}) 
    d {f}_{\text{PoIs}} d {y}_{A}
\end{align}

Recall that the posterior probability of $\bm{f}_{\text{PoIs}} \mid X_{A}, \bm{y}_{A} $ is still Gaussian. The entropy is  
\begin{equation}
     H(\bm{f}_{\text{PoIs}} \mid X_A, \bm{y}_{A}) = \frac{1}{2} \log \abs{\Sigma_{\bm{f}_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{x}_{A}}}+\frac{\abs{V_{\text{PoIs}}}}{2}(\log (2\pi) + 1), 
\end{equation}
where $\Sigma_{\bm{y}_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{x}_{A}}$ can be computed using Eq. \eqref{eq:posterior_covariance_deterministic}. 


\subsection{Airdrop Process}
\todo{explain how UAV drops a sensor (hover or with velocity); how sensor moves after being dropped; why do we make the Gaussian assumption}

The trajectory of the sensor affected by the wind can be modeled using \textcolor{red}{XXX}. In the paper, when the UAV is throwing the sensor, it is assumed to be steady. The initial velocity $(\dot{x}^{sensor},\dot{y}^{sensor}, \dot{z}^{sensor})$ of the sensor is zero. The horizontal motion can be modeled as
\begin{align}
    \begin{aligned}
        x^{sensor}_{t+1} =  x^{sensor}_{t} + W_x (p_{i,t}, z^{sensor}_{t})T
    \end{aligned} \\
    \begin{aligned}
        y^{sensor}_{t+1} =  y^{sensor}_{t} + W_y (p_{i,t},  z^{sensor}_{t})T
    \end{aligned}
\end{align}
where $(W_x, W_y)$ is the wind speed in the $x$ and $y$ directions and $T$ is the time step.

The vertical motion can be modeled as 
\begin{equation}
    \small
    \begin{bmatrix}
       z^{sensor}_{t+1} \\ 
       \dot{z}^{sensor}_{t+1}
    \end{bmatrix} =
    \begin{bmatrix}
       z^{sensor}_{t} + \dot{z}^{sensor}_{t}T - \frac{1}{2}(g - \frac{1}{2m_c} \rho \kappa ({\dot{z}^{sensor}_{t}})^2) T^2 \\ 
       \dot{z}^{sensor}_{t+1} - (g - \frac{1}{2m_c} \rho \kappa ({\dot{z}^{sensor}_{t}})^2) T
    \end{bmatrix}
\end{equation}
where $g$ is the gravitational acceleration, $m_c$ is the mass of sensors, $\rho$ is the density of air, and $\kappa$ is the surface coefficient of sensors.

\section{Problem Formulation}
In this section, we formulate the path planning problem for UAV sensor airdrop missions. 
%Our objective is to find a tour for the UAV to drop sensors considering the budget constraint (e.g., battery capacity) and the stochastic landing locations of sensors.
%Our objective is to determine the optimal path, drop points, and drop angles considering constraints of airdrop dynamics, underwater conditions, and battery size. By formulating the mission as an offline optimization problem, we aim to maximize mission efficiency and sensor coverage. 

 %A UAV is equipped with a size $B$ battery and $n$ sensors, denoted by the set $\bm{N}=\{1,2,\ldots, N\}$. 
 The mission of budget-constrained UAV is to plan an optimal route $\tau^*$ and airdrop the $N$ sensors, indexed by the set $\mathcal{N}=\{1,2,\ldots, N\}$, to an area on the ground to measure $m$ distinct Points of  Interest (PoIs). We assume that UAV can drop the sensors at some discretized locations in the air and all the possible airdrop locations form a complete metric graph $G=(V_{\text{airdrop}}, E)$, where $V_{\text{airdrop}}$ denotes the collection of all possible airdrop locations and $E$ denotes the set of possible transitions between airdrop locations. Each edge $e_{ij}$ has a corresponding cost $c_{ij}$. The cost function is given by $\frac{d_{ij}}{s}$
\iffalse
 \begin{equation} c_{ij} = 
     \begin{cases}
     d_{ij}/s & \text{ if node $i$ and node $j$ are connected} \\ 
     \infty& \text{ else} 
    \end{cases}
\end{equation}
\fi
where $d_{ij}$ is the flight distance between vertex $v_i$ and vertex $v_j$ and $s$ is the constant spend of the UAV. The UAV can travel between the nodes on the graph $G$ and the distance must not exceed the UAV’s battery capacity $B$. For simplicity, we confine our discussion to the case where the UAV can drop one sensor at one vertex. The formulation can be easily generalized to the case where we can drop multiple sensors at one vertex. 

When the sensor landing location is deterministic, the problem is similar to the classic sensor placement problem with budget constraints. A good airdrop route would result in a set of landing locations, denoted as $A$, that maximize the difference between $H(\bm{f}_{\scaleto{\text{PoIs}}{4pt}})$ and $H(\bm{f}_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{X}_{A}, \bm{y}_{A})$, i.e.,  uncertainty reduction at $V_{\text{PoIs}}$. However, due to the disturbances of the wind, the landing position $\mathbf{x}_v$ when a sensor is dropped at the node $v$ is stochastic. That is, the location where the sensor will take measurements is stochastic. In such a case, we are interested in expected uncertainty reduction at $V_{\text{PoIs}}$, i.e.,  $H(\bm{f}_{\scaleto{\text{PoIs}}{4pt}}) - \mathbb{E} [{H(\bm{f}_{\scaleto{\text{PoIs}}{4pt}} \mid \mathbf{X}_{A}, \bm{y}_{A})}]$.

% Mathematically, we want to find

%\argmax_{A \subseteq V_{\text{sensor}}} MI(\bm{f}_{\scaleto{\text{PoIs}}{4pt}}, ~\bm{f}_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{X}_{A}, \bm{y}_{A})
%It should be noted that the objective in Eq. \eqref{eq:mutual_information_objective} is the mutual information (MI) between $\bm{f}_{\scaleto{{\text{PoIs}}}{4pt}}$ and $\bm{f}_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{X}_{A}, \bm{y}_{A}$, i.e., $I(\bm{f}_{\scaleto{{\text{PoIs}}}{4pt}}, ~\bm{f}_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{X}_{A}, \bm{y}_{A})$.


At a high level, the problem studied in this paper is stated below.

\textbf{Problem}. 
%Given a discrete undirected graph $G=(V_{\text{airdrop}},E)$, an associated edge cost function $C$, $N$ sensors, and $m$ PoIs, find the optimal route $\tau^* = (\tau_1, \tau_2, ..., \tau_w), \tau_i =(t,v_j) \in [t_0,t_{end}] \times V $, the optimal drop points $A =[A_1, A_2, ..., A_N] \subseteq V_{airdrop}$, and the optimal drop angles $\bm{\theta} = [\bm{\theta}_1, \bm{\theta}_2, ..., \bm{\theta}_N], \bm{\theta}_j \in [0, 2 \pi)$ to minimize the cost function, such that 
Given a discrete undirected graph $G=(V_{\text{airdrop}},E)$, an associated edge cost function $C$, $N$ sensors, and $m$ PoIs, find the optimal route $\tau^* = (v_1, v_2, ..., v_{\abs{\tau^*}})$ and drop one sensor in each vertex $v_i \in \tau^*$ to maximize the expected uncertainty reduction at PoIs. Mathematically, 
\begin{align}
    \max_{{\tau}} & ~H(\bm{f}_{\scaleto{\bm{V}_{\text{PoIs}}}{4pt}}) - \mathbb{E} [H(\bm{f}_{\scaleto{\text{PoIs}}{4pt}} \mid  \mathbf{X}_{A}, \bm{y}_{A})]  \\
    \text{s.t.} &~C(\tau) \leq B, 
\end{align}
where the expected conditional entropy can be computed as 
\begin{align}\label{eq:expected_conditional_entropy}
    &\int \int H(f_{\scaleto{\text{PoIs}}{4pt}} \mid y_{A}) p(y_A \mid \mathbf{x}_{A})p(\mathbf{x}_{A}) ~\text{d} {y}_{A} ~\text{d} \mathbf{x}_{A}.
   % =& \int H(f_{\scaleto{\text{PoIs}}{4pt}} \mid {y}_{A}) p(\bm{x}_{A}) ~\text{d} \bm{x}_{A}
\end{align}

\iffalse
The goal is to select $N$ vertices in graph $G$ to drop sensors to reduce the uncertainty of PoIs. We denote the set of PoIs as $V_{\text{POIs}}$. Mathematically, 
\begin{align}
    \max_{A \subseteq V_{sensor}} H(\bm{f}_{\scaleto{\text{PoIs}}{4pt}}) -  H(\bm{f}_{\scaleto{\text{PoIs}}{4pt}} \mid X_A,\bm{y}_{A}),
\end{align}


where $H(f(\mathcal{P}))$ is the entropy of the prior distribution (Gaussian) of values of PoIs and can be computed analytically; $\mathbb{E} \left [ H(f_{\mathcal{P}} \mid \mathcal{L}(A)) \right ]$ denotes the expected entropy of the posterior distribution of values of PoIs when a set of sensors $A$ is dropped. 

The challenge is to compute $\mathbb{E} \left [ H(f_{\mathcal{P}} \mid \mathcal{L}(A)) \right ]$.
we need to solve the following integral:
\begin{equation}\label{problem:main_original}
    \int \int H(f_\mathcal{P} \mid \mathcal{L}(A), y)p(y \mid \mathcal{L}(A))p(\mathcal{L}(A)) ~\text{d} y ~\text{d} \mathcal{L}(A).
\end{equation}
\fi

\todo{When the input location is uncertain, the resulting process is in general no longer a GP and the posterior distribution is in general not a Gaussian, rendering the optimization problem intractable.}   We have to resort to approximation. The challenge here originates from the stochasticity of the landing positions of the sensors. Even if the input location uncertainty i.i.d. Gaussian, the resulting function values at different locations at not necessarily jointly Gaussian, making the computation of the posterior distribution intractable.  In the following section, we will introduce a way of directly approximating the objective to one deterministic objective and show the approximated problem can be solved nearly optimally.   

\subsection{Relaxation of Stochastic Case: Expected Mean and Covariance Function \todo{Ahmad}}
\todo{this part should explain the logical reasoning for using this type of approximation. After approximation, it is a deterministic problem. }

\todo{check notation in Sec. \ref{sec:notation}}


We assume that $\mathbf{x}_v$ has a Gaussian distribution with a known mean $\mu_{\mathbf{x}_v}$ and variance $\sigma_{\mathbf{x}_v}^2$.


%%%
\iffalse
The idea of approximating the problem \todo{XX} is to `propagate' the uncertainty of the input to the output such that the resulting problem is similar to problem \todo{XX} but with a different output uncertainty. 

\subsection{Relaxation of Stochastic Case I: Linearizing the Output}
Based on \cite{mchutchon2011gaussian}, 
\begin{equation}
    \bm{f}(\bar{\bm{x}} + \bm{\epsilon}_{\bm{x}}) = \bm{f}(\bar{\bm{x}})+ \frac{\partial \bm{f}(\bar{\bm{x}})}{\partial \bar{\bm{x}}}^T \bm{\epsilon}_{\bm{x}}+\ldots
\end{equation}

If we limit our approximation accuracy to the first order in trade for computational tractability, we get a linear model to propagate the input noise to the output:
\begin{equation}
    \bm{y} = \bm{f}(\bm{x}) + \bm{\partial}_{\bar{f}}^T \bm{\epsilon}_{\bm{x}}+\epsilon_y.
\end{equation}
where both  $\epsilon_x \sim \mathcal{N}(0, \sigma^2_{\epsilon_x})$ and $\epsilon_y \sim \mathcal{N}(0, \sigma^2_{\epsilon_y})$ are i.i.d. Gaussian Noise; $\bm{\partial}_{\bar{f}}$ represents the slope of function at the center of $\bm{x}$.  The probability of an observation $y$ is, therefore,
\begin{equation}
    p(\bm{y} \mid \bm{f}) = \mathcal{N}(\bm{f}, \sigma_y^2+\bm{\partial}_{\bar{f}}^T\sigma_{x}^2\bm{\partial}_{\bar{f}} ). 
\end{equation}


Combing with the Gaussian prior $p(\bm{f} \mid {\bm{x}_*,\mathcal{D}}) = \mathcal{N}(\bar{\bm{f}}, \text{Cov}({\bm{f}}))$, the predictive posterior distribution is still a Gaussian with mean and variance as 

\begin{align}
    \begin{aligned}
        \bm{\bar{f}} = \mu(x_*) + {k}(\bm{x}_*, {X})  [ k({X}, {X}) + \sigma^2_yI \\+\text{diag}\{ \Delta_{\bar{f}} \Sigma_{x} \Delta_{\bar{f}}^T \}  ]^{-1}(\bm{y} - \mu(X))
    \end{aligned}\\
    \begin{aligned}
        \text{Cov}(\bm{f}) = k(\bm{x}_*, \bm{x}_*)-k(\bm{x}_*, X)^T[k(X, X)+ \\ \sigma_y^2 I+ \text{diag}\{ \Delta_{\bar{f}} \Sigma_{x} \Delta_{\bar{f}}^T \}]^{-1}k( \bm{x}_*,X)
    \end{aligned}
\end{align}

\fi

A good placement would maximize the different between $H(\bm{f}_{\scaleto{\text{PoIs}}{4pt}})$ and $H(\bm{f}_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{X}_{A}, \bm{y}_{A})$, i.e., reduce the uncertainty at $V_{\text{PoIs}}$. Mathematically, we want to find
\begin{align}\label{eq:mutual_information_objective}
    A^* & =  \argmax_{A \subseteq V_{\text{sensor}}} H(\bm{f}_{\scaleto{{\text{PoIs}}}{4pt}}) - H(\bm{f}_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{X}_{A}, \bm{y}_{A}).
\end{align}
%\argmax_{A \subseteq V_{\text{sensor}}} MI(\bm{f}_{\scaleto{\text{PoIs}}{4pt}}, ~\bm{f}_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{X}_{A}, \bm{y}_{A})
It should be noted that the objective in Eq. \eqref{eq:mutual_information_objective} is the mutual information (MI) between $\bm{f}_{\scaleto{{\text{PoIs}}}{4pt}}$ and $\bm{f}_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{X}_{A}, \bm{y}_{A}$, i.e., $I(\bm{f}_{\scaleto{{\text{PoIs}}}{4pt}}, ~\bm{f}_{\scaleto{\text{PoIs}}{4pt}} \mid \bm{X}_{A}, \bm{y}_{A})$.


